Practical Secure Aggregation for Federated Learning on User-Held Data

Secure Aggregation protocols allow a collection of mutually distrust parties, each holding a private value, to collaboratively compute the sum of those values without revealing the values themselves. We consider training a deep neural network in the Federated Learning model, using distributed stochastic gradient descent across user-held training data on mobile devices, wherein Secure Aggregation protects each user's model gradient. We design a novel, communication-efficient Secure Aggregation protocol for high-dimensional data that tolerates up to 1/3 users failing to complete the protocol. For 16-bit input values, our protocol offers 1.73x communication expansion for $2^{10}$ users and $2^{20}$-dimensional vectors, and 1.98x expansion for $2^{14}$ users and $2^{24}$ dimensional vectors.

==> SecAgg2016.Abstract.tex <==
We design a novel, communication-efficient Secure Aggregation protocol for
high- dimensional data that tolerates up to $\frac{1}{3}$ users failing to
complete the protocol.  For $2^{20}$-dimensional vectors of 16-bit input
values,  our protocol offers $1.73\times$ communication expansion for $2^{10}$
users and $3.62\times$ expansion for $2^{14}$ users. As motivation, we
consider training a deep neural network in the Federated Learning model, using
distributed gradient descent across user-held training data on mobile devices,
wherein Secure Aggregation protects each user's model gradient.

